Reproducibility and Artifact Consistency of the SIGIR 2022 Recommender Systems Papers Based on Message Passing

Graph-based techniques relying on neural networks and embeddings have gained attention as a way to develop Recommender Systems (RS) with several papers on the topic presented at SIGIR 2022 and 2023. Given the importance of ensuring that published research is methodologically sound and reproducible, in this paper we analyze 10 graph-based RS papers, most of which were published at SIGIR 2022, and assess their impact on subsequent work published in SIGIR 2023. Our analysis reveals several critical points that require attention: (i) the prevalence of bad practices, such as erroneous data splits or information leakage between training and testing data, which call into question the validity of the results; (ii) frequent inconsistencies between the provided artifacts (source code and data) and their descriptions in the paper, causing uncertainty about what is actually being evaluated; and (iii) the preference for new or complex baselines that are weaker compared to simpler ones, creating the impression of continuous improvement even when, particularly for the Amazon-Book dataset, the state-of-the-art has significantly worsened. Due to these issues, we are unable to confirm the claims made in most of the papers that we examined and attempted to reproduce.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/article_template.tex <==
\clearpage
\section{New algorithm}
\citet{newalgorithm} presents \emph{newalgorithm} (ALGNAME), ...


\subsection{Datasets} 
The evaluation is performed on the datasets described and processed as follows, their statistics are reported in Table \ref{tab:ALGNAME_dataset}

\begin{description}
\item[dataset:] 
\end{description}


\begin{table}[h]
    \begin{tabular}{lcccc}
    \toprule
    Dataset			& Interactions	& Items		& Users 	& Sparsity	\\
    \midrule
    dataset	 	& -	 		& -		& -		& - 	\\
    dataset	 	& -	 		& -		& -		& - 	\\
	\bottomrule
   	\end{tabular}
    \caption{Dataset characteristics for ALGNAME.}
    \label{tab:ALGNAME_dataset}
\end{table}

% \begin{table}
%     \begin{tabular}{l|ccccccc|}
%     \toprule
%                &  Pop max &  Pop min &  Pop mean &  Pop median &  Gini Index &  Kendall Tau &  Shannon Entropy &  Herfindahl Index \\
%     \midrule
%     dataset	    & -	    & -	    & -	    & -	    & -	    & -\\
%     \bottomrule
%     \end{tabular}
%     \caption{Dataset popularity bias characteristics.}
%     \label{tab:CMN_dataset_popularity}
% \end{table}

\paragraph{Checklist:}
\begin{itemize}
    \item The characteristics of the data are consistent with the description in the paper?
\end{itemize}



\subsection{Evaluation protocol}
\begin{description}
    \item[Data split:] The data splitting is performed in the following way:
    
    \item[Reported metrics:] The metrics reported are:
    
    \item[The original train-test split of the data is available on the Github repository?]  \footnote{\url{URL HERE}}.
    
    \item[(If required) The original negative item split used for the evaluation is available on the Github repository?]
    
    \item[The provided data splits have a distribution consistent with the split described?] 
    
    \item[Does the paper mention a validation set?] 
    
    \item[Is it stated that the evaluation is performed in the same way (data, metrics) as another article?]     
\end{description}


\subsection{Baselines}
The paper reports the following baselines:

\begin{description}
\item[baseline:] 
\end{description}


\paragraph{Checklist:}
\begin{itemize}
    \item Are simple methods like ItemKNN, UserKNN etc among the baselines?    
\end{itemize}




\subsection{Hyperparameter tuning} 
\begin{description}
    \item[Validation data:] The hyperparameters are tuned using a validation set? (or not described in the paper)
    
    \item[Optimized metric:] The search optimizes metric... 
    
    \item[Tuning method:] The search is performed with (grid search/random/manual...)
    
    \item[Hyperparameters range and distribution:] 
    
    \item[Number of epochs:] The number of epochs is selected with earlystopping... / not specified
    
    \item[Hyperparameters of baselines:] The hyperparameter for the baselines are searched... are taken from the original papers... 

    \item[Consistency of the optimal hyperparameters of reproduced method:] The optimal hyperparameter for the reproduced method are reported in  Table \ref{tab:ALGNAME_hyperparameter_values}. They are/not consistent with the search space.
\end{description}

\begin{table}[h]
    \begin{minipage}{\textwidth}
    \centering
    \footnotesize
    \begin{tabular}{lcc}
    \toprule
    Hyperparameter	& Described in	& \multicolumn{1}{c}{Value}	\\
                	&               & All datasets	\\    
    \midrule
    name	 	& Paper / source code	    & -  	\\
    name	 	& Paper / source code		& -	 	\\
    name	 	& Paper / source code		& -	 	\\
	\bottomrule
   	\end{tabular}
   	\end{minipage}
    \caption{Hyperparameter Values}
    \label{tab:ALGNAME_hyperparameter_values}
\end{table}






\subsection{Source code} 
The source code is publicly available\footnote{\url{TODO}}.
\begin{description}
    \item[Is the original source code executable with at most minor changes?]
    
    \item[In the original source code is the test data used during the training in any way?]
    
    \item[Are there inconsistencies between the source code and what described in the paper?] (for example the architecture or the implementation o the BPR loss)
\end{description}




\subsection{Outcome} 
\begin{description}
     \item[Is it possible to reproduce the results reported in the paper?] 
\end{description}
    



\subsection{Methodological considerations}

On Github t..









\tableArticleResult{ALGNAME}{ALGNAME}{movielens1m}{Movielens 1M}{0}
\tableArticleResult{ALGNAME}{ALGNAME}{amazon_music}{Amazon Music}{0}


\tableTime{ALGNAME}{ALGNAME}{movielens1m}{Movielens 1M}
\tableTime{ALGNAME}{ALGNAME}{amazon_music}{Amazon Music}

\tableHyperParams{ALGNAME}{ALGNAME}{KNN}
\tableHyperParams{ALGNAME}{ALGNAME}{ML_graph}
\tableHyperParams{ALGNAME}{ALGNAME}{neural}






==> sections/dataset_commonality.tex <==
\clearpage

\section{Which articles use the same data split}


\begin{table}[h]
    \caption{Which articles use the same data split Amazon Book.}
    \footnotesize
    \centering

\begin{tabular}{llllllll}
\toprule
{} & GTN &   HCCF &   INMO &   KGCL & LightGCN &   RGCF & SimGCL \\
\midrule
GTN      &   - &  False &  False &  False &     \textcolor{red}{\textbf{True}} &  False &   \textcolor{red}{\textbf{True}} \\
HCCF     &   - &      - &  False &  False &    False &  False &  False \\
INMO     &   - &      - &      - &  False &    False &  False &  False \\
KGCL     &   - &      - &      - &      - &    False &  False &  False \\
LightGCN &   - &      - &      - &      - &        - &  False &   \textcolor{red}{\textbf{True}} \\
RGCF     &   - &      - &      - &      - &        - &      - &  False \\
SimGCL   &   - &      - &      - &      - &        - &      - &      - \\
\bottomrule
\end{tabular}
   
\end{table}




\begin{table}[h]
    \caption{Which articles use the same data split Yelp 2018.}
    \footnotesize
    \centering

\begin{tabular}{lllllllll}
\toprule
{} & GTN &   HAKG &   HCCF &   INMO &   KGCL & LightGCN &   RGCF & SimGCL \\
\midrule
GTN      &   - &  False &  False &  False &  False &     \textcolor{red}{\textbf{True}} &  False &   \textcolor{red}{\textbf{True}} \\
HAKG     &   - &      - &  False &  False &   \textcolor{red}{\textbf{True}} &    False &  False &  False \\
HCCF     &   - &      - &      - &  False &  False &    False &  False &  False \\
INMO     &   - &      - &      - &      - &  False &    False &  False &  False \\
KGCL     &   - &      - &      - &      - &      - &    False &  False &  False \\
LightGCN &   - &      - &      - &      - &      - &        - &  False &   \textcolor{red}{\textbf{True}} \\
RGCF     &   - &      - &      - &      - &      - &        - &      - &  False \\
SimGCL   &   - &      - &      - &      - &      - &        - &      - &      - \\
\bottomrule
\end{tabular}
   
\end{table}





\begin{table}[h]
    \caption{Which articles use the same data split Gowalla.}
    \footnotesize
    \centering

\begin{tabular}{lllll}
\toprule
{} & GDE &    GTN &   INMO & LightGCN \\
\midrule
GDE      &   - &  False &  False &    False \\
GTN      &   - &      - &  False &     \textcolor{red}{\textbf{True}} \\
INMO     &   - &      - &      - &    False \\
LightGCN &   - &      - &      - &        - \\
\bottomrule
\end{tabular}
   
\end{table}







\begin{table}[h]
    \caption{Which articles use the same data split Movielens 1M.}
    \footnotesize
    \centering

\begin{tabular}{lll}
\toprule
{} & GDE &   RGCF \\
\midrule
GDE  &   - &  False \\
RGCF &   - &      - \\
\bottomrule
\end{tabular}
   
\end{table}




\begin{table}[h]
    \caption{Which articles use the same data split LastFM.}
    \footnotesize
    \centering

\begin{tabular}{lll}
\toprule
{} & GTN &  HAKG \\
\midrule
GTN  &   - &  \textcolor{red}{\textbf{True}} \\
HAKG &   - &     - \\
\bottomrule
\end{tabular}
   
\end{table}







==> sections/methodology.tex <==
\clearpage
\section{Introduction}
\mf{Questa sezione e' dal vecchio documento del 2019}

In recent years there has been significant interest in applying deep learning techniques (DL) to recommender systems, with many successful results in various domains.
Deep learning is known to provide the most benefits for non structured data sources and when a huge amount of data is available. For smaller and structured data sources its advantage over traditional techniques may either be small or disappear completely.
In this paper we look at two recent papers proposing DL recommenders and compare their results with properly tuned non DL baselines.

\section{Methodology and Baselines}
\label{sec:our_evaluation}
We considered the following baseline methods in our experiments, all of which are conceptually simple.
\begin{description}
\item[TopPopular:]
A non-personalized method that recommends the most popular items to everyone. Popularity is measured by the number of explicit or implicit ratings.
\end{description}

\subsection{KNN}
\begin{description}
\item[ItemKNN:]
A traditional Collaborative-Filtering (CF) approach based on $k$-nearest-neighborhood (KNN) and item-item similarities \cite{wang2006unifying}. We used various similarities as listed in Section \ref{sec:similarity}.
% We used the cosine similarity $s_{ij}$ between items $i$ and $j$ computed as
% \begin{equation}
% \label{eqn:cosine_similarity}
% s_{ij} = \frac{\vec{r}_i \cdot \vec{r}_j}{\| \vec{r}_i\| \| \vec{r}_j\| + h}
% \end{equation}
% where vectors $\vec{r}_i, \vec{r}_j \in \mathbb{R} ^ {|U|}$ represent the implicit ratings of a user for items $i$ and $j$, respectively, and
% $|U|$ is the number of users.
% Ratings can be optionally normalized (weighted) either with TF-IDF or BM25, as described in \cite{wang2008probabilistic}.
% Parameter $h$ (the \emph{shrink term}) is used to lower the similarity between items having only few interactions \cite{bell2007improved}.
The hyperparameters of the method are those of the specific similarity and the neighborhood size $k$.

\item[UserKNN:]
A neighborhood-based method using collaborative user-user similarities.
Hyperparameters are the same as used for ItemKNN \cite{sarwar2001item}.
% TODO: check reference.

\item[ItemKNN-CBF:]
A neighborhood content-based-filtering (CBF) approach with item similarities computed by using item content features (attributes).We used various similarities as listed in Section \ref{sec:similarity}.
% %The similarity between items is computed as
% \begin{equation}
% \label{eqn:cosine_similarity2}
% s_{ij} = \frac{\vec{f}_i \cdot \vec{f}_j}{\| \vec{f}_i\| \| \vec{f}_j\| + h}
% \end{equation}
% where vectors $\vec{f}_i, \vec{f}_j \in \mathbb{R} ^ {|F|}$ describe the features of items $i$ and $j$, respectively, and
% $|F|$ is the number of features.
% Features can be optionally weighted either with TF-IDF or BM25.
The hyperparameters are the same used for ItemKNN \cite{lops2011content}.

\item[ItemKNN-CFCBF:]
% TODO: rephrased, please check.
A hybrid CF+CFB algorithm based on item-item similarities.
The similarity is computed by first concatenating, for each item $i$, the vector of ratings and the vector of features --
$\left[ \vec{r}_i \, , w \vec{f}_i \right]$ -- and by later computing the cosine similarity \label{eqn:cosine_similarity2} between the concatenated vectors.
Hyper-parameters are the same used for ItemKNN, plus a parameter $w$ that weights the content features with respect to the ratings.
%A neighborhood-based approach based on item-to-item similarities computed as in ItemKNN-CBF. The similarity is computed by considering as item features both the original content features and the users who have that item in their profile. This algorithm is therefore a hybrid CF-CBF. It has the same parameters as ItemKNN-CBF and a weight to be applied to the content features.

\item[\palpha :]

A simple graph-based algorithm which implements a random walk between users and items \cite{cooper2014P3alpha}.
%Each user is connected to the items he or she interacted with and each item is connected to the users in the same way.
Items for user $u$ are ranked based on the probability of a random walk with three steps starting from user $u$.
The probability $p_{ui}$ to jump from user $u$ to item $i$ is computed from the implicit user-rating-matrix as
$p_{ui} = \left( r_{ui} / N_u \right) ^\alpha $, where $r_{ui}$ is the rating of user $u$ on item $i$, $N_u$ is the number of ratings of user $u$ and $\alpha$ is a dumping factor.
The probability $p_{iu}$ to jump backward is computed as $p_{iu} = \left( r_{ui} / N_i \right) ^\alpha $, where $N_i$ is the number of ratings for item $i$.
The method is equivalent to an KNN item-based CF algorithm, with the similarity matrix defined as
\begin{equation}
\label{eqn:p3a}
s_{ij} = \sum_v{ p_{jv} p_{vi} }
\end{equation}

The parameters of the method are the numbers of neighbors $k$ and the value of $\alpha$.
We include this algorithm as a baseline because it provides good recommendation quality at a low computational cost.
\item[\pbeta :]
A version of \palpha~proposed in \cite{paudel2017Rp3beta}. Here, the outcomes of \palpha~are modified by dividing the similarities by each item's popularity raised to the power of a coefficient $\beta$. If $\beta$ is 0, the algorithm is equivalent to \palpha.
Its parameters are the numbers of neighbors $k$ and the values for $\alpha$ and $\beta$.
\end{description}



\subsection{Similarity heuristics}
\label{sec:similarity}
In this section we list all the similarities we used in the KNN models. We adopt the following notation, vectors $\vec{r}_i, \vec{r}_j \in \mathbb{R} ^ {|U|}$ represent the ratings of a user for items $i$ and $j$, respectively, and $|U|$ is the number of users. In case of CBF recommenders the similarity will be computed using feature vectors $\vec{f}_i, \vec{f}_j \in \mathbb{R} ^ {|F|}$, where  $|F|$ is the number of features. All equations are written with rating vectors but can be seamlessly applied to CBF algorithms by using feature vectors instead.

Rating vectors and feature vectors can be optionally normalized (weighted) either with TF-IDF or BM25, as described in \cite{wang2008probabilistic}. In case of a CBF model, the weighting is applied to the features, in case of a CF model it is applied on the items.

Hyperparameter $h$ (the \emph{shrink term}) is used to lower the similarity between items having only few interactions, or features, in common \cite{bell2007improved}.


\begin{description}
\item[Cosine] The cosine similarity $s_{ij}$ between items $i$ and $j$ is computed as follows:
\begin{equation}
\label{eqn:cosine_similarity}
s_{ij} = \frac{\vec{r}_i \cdot \vec{r}_j}{\| \vec{r}_i\| \| \vec{r}_j\| + h}
\end{equation}

\item[Asymmetric Cosine] Proposed by \cite{aiolli2013AsymmetricCosine} , adds an exponentiation operation on the norms of the two vectors.
\begin{equation}
\label{eqn:asymmetric_cosine_similarity}
s_{ij} = \frac{\vec{r}_i \cdot \vec{r}_j}{\| \vec{r}_i\|^\alpha \| \vec{r}_j\|^{1-\alpha} + h}
\end{equation}

\item[Dice - S{\o}rensen] Is a similarity measure on sets, therefore defined on boolean vectors. Given two sets or verctors the respective Dice similarity can be computed as a linear function of Jaccard similarity and vice versa. The Dice coefficient doesn't satisfy the triangle inequality, it can be considered a semimetric version of the Jaccard index.
\begin{equation}
\label{eqn:dice_similarity_set_notation}
s_{AB} = 2 \frac{A \cap B}{\|A \| + \|B\| + h}
\end{equation}
\begin{equation}
\label{eqn:dice_similarity}
s_{ij} = 2 \frac{\vec{r}_i \cdot \vec{r}_j}{\| \vec{r}_i\| + \| \vec{r}_j\| + h}
\end{equation}


\item[Jaccard - Tanimoto] Is a similarity measure on sets, therefore defined on boolean vectors. The term Tanimoto is sometimes used to refer to its formulation on vectors, however the corresponding similarity is not a proper similarity since its distance does not preserve the triangle inequality.
\begin{equation}
\label{eqn:jaccard_similarity_set_notation}
s_{AB} = \frac{A \cap B}{\|A \| + \|B\| - \|A \cap B\| + h}
\end{equation}

\begin{equation}
\label{eqn:jaccard_similarity}
s_{ij} = \frac{\vec{r}_i \cdot \vec{r}_j}{\| \vec{r}_i\| + \| \vec{r}_j\| - \vec{r}_i \cdot \vec{r}_j + h}
\end{equation}


\item[Tversky]
Is an asymmetric similarity measure on sets which is a generalisation of Dice/S{\o}rensen and Tanimoto/Jaccard coefficients.
\begin{equation}
\label{eqn:tversky_similarity_set_notation}
s_{AB} = \frac{A \cap B}{\|A \cap B\| + \alpha\|A - B\| + \beta\|B - A\| + h}
\end{equation}
Where $-$ denotes the \emph{relative complement} of two sets, therefore $\|B - A\|$ means the number of elements in B that are not in A and can be represented as $\|B\| - \|A \cap B\|$ . 
If $\alpha = \beta = 1$ we get the Tanimoto coefficient, if $\alpha = \beta = 0.5$ we get the Dice coefficient.

In case of boolean attributes it can be calculated as follows:
\begin{equation}
\label{eqn:tversky_similarity}
s_{ij} = \frac{\vec{r}_i \cdot \vec{r}_j}{\vec{r}_i \cdot \vec{r}_j + \alpha(\| \vec{r}_i\| - \vec{r}_i \cdot \vec{r}_j) + \beta(\| \vec{r}_j\| - \vec{r}_i \cdot \vec{r}_j) + h}
\end{equation}


\end{description}







\subsection{SLIM}
\begin{description}
\item[SLIM ElasticNet:] A SLIM \cite{ning2011SLIM} variant proposed by \cite{levy2013SLIM_ElasticNet} which learns the Item similarity matrix one item at a time (e.g. one column $w$ at a time) by solving a regression problem in such a way that the interactions for the target item $y$ are learned by using all other interactions as training data, $X$. To implement \emph{SLIM ElasticNet} we used a standard ElasticNet solver provided in the \small{\texttt{scikit-learn}} \normalsize package for Python\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.linear_model.ElasticNet.html}}. The model optimises the following objective function:
\begin{equation}
\label{eqn:SLIM_elasticnet}
\operatornamewithlimits{argmin} \limits_{W}\frac{1}{2 \cdot n\_samples} \normF{y - Xw} + \alpha \cdot l1\_ratio \norm{w}
+ \frac{\alpha}{2} \cdot \left( 1 - l1\_ratio\right) \cdot  \normF{w}
\end{equation}
Where $\alpha$ is a constant that multiplies the penalty terms and controls their magnitude with respect tot the error component and l1\_ratio is the prevalence of l1 over l2 regularization.


\item[SLIM BPR:] A SLIM \cite{ning2011SLIM} variant which optimizes BPR instead of MSE \cite{Balog2019SLIMBPR,Suglia2017SLIMBPR,Anelli2017SLIMBPR}.

\end{description}

\subsection{Matrix Factorization}

\subsubsection{Mathematical notation}
In order to describe the MF baselines we adopt the following notation. $U$ is the set of users and $|U|$ their number, similarly $I$ is the set of items and $|I|$ their number, $f \in F$ is the index of the latent factor whose total number is $|F|$; $W \in \mathbb{R} ^ {|U|x|F|}$ is a two-dimensional matrix containing the user factors and $H \in \mathbb{R} ^ {|I|x|F|}$ is a two-dimensional matrix containing the item factors.
$R \in \mathbb{R} ^ {|U|x|I|}$ is the rating matrix.

\subsubsection{PureSVD}
A simple matrix factorization method described in \cite{cremonesi2010performance}.
To implement \emph{PureSVD}, we use a standard SVD decomposition provided in the \small{\texttt{scikit-learn}} \normalsize package for Python (\small{\texttt{sklearn.utils.extmath.randomized\_svd}}\normalsize). Latent factors may be either positive or negative. \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.utils.extmath.randomized_svd.html}} 
\mf{thanks to folding-in it is equivalent to FISM and so to item-KNN \cite{cremonesi2010performance}}

\subsubsection{Non-negative MF (NMF or NNMF):} Non Negative MF \cite{cichocki2009fastNMF} guarantees all latent factors to be positive, a constraint SVD does not have. We use a standard NMF decomposition provided in the \small{\texttt{scikit-learn}} \normalsize package for Python (\small{\texttt{sklearn.decomposition.NMF}}\normalsize). NMF decomposition is not unique.




\subsubsection{FunkSVD}
The original MF algorithm described by Simon Funk \footnote{\url{http://sifter.org/~simon/journal/20061211.html}}. This model optimized MSE and is best suited for rating prediction.

The model optimizes the following:
\begin{equation}
\operatornamewithlimits{argmin} \limits_{W,H}\frac{1}{2} \norm{R - WH^T - \mu - B_I - B_U} + \mbox{F reg.} %\frac{\lambda}{2}\left(\normF{W} + \normF{H}\right)
\label{model:FunkSVD}
\end{equation}


The prediction is computed as follows:
$$  \hat{r}_{ui} = \mu + b_u + b_i + \sum^{|F|}_{f} W_{u,f} \cdot H_{i,f}  $$

Where $\mu$ is the global bias, $b_u \in \mathbb{R} ^ {|U|}$ the user bias, $b_i \in \mathbb{R} ^ {|I|}$ the item bias. $\mbox{F reg.}$ refers to the latent factors regularisation with Frobenius norm $\frac{\lambda}{2}\left(\normF{W} + \normF{H}\right)$




\subsubsection{BPRMF}
Matrix factorisation algorithm optimising BPR \cite{rendle2009bprMF}\footnote{\url{https://arxiv.org/ftp/arxiv/papers/1205/1205.2618.pdf}} proposed for implicit feedback. \mf{add bpr optimization?}
The prediction is computed as follows:
$$  \hat{r}_{ui} = \sum^{|F|}_{f} W_{u,f} \cdot H_{i,f} $$









\subsubsection{AsymmetricSVD} \mf{very slow, I can try it but as the last after the other experiments are concluded. For some datasets it may not be feasible (>1 day per each case)}



\subsubsection{Implicit Alternating Least Squares (IALS)} 
IALS \cite{hu2008IALS} \footnote{\url{http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.167.5120&rep=rep1&type=pdf}} is an evolution of ALS to handle implicit interactions and can handle different types of them. Interactions are transformed into a value of \emph{confidence}.

\begin{equation}
\operatornamewithlimits{argmin} \limits_{W,H}\frac{1}{2} \norm{C \left(P - WH^T\right)} + \mbox{F reg.} %\frac{\lambda}{2}\left(\normF{W} + \normF{H}\right)
\label{model:IALS}
\end{equation}

Where $C \in \mathbb{R}^ {|U|x|I|}$ is the \emph{confidence} matrix, computed from $R$, and $P \in \mathbb{Z} [0, 1]$ is the \emph{preference} matrix, obtained by binarising $R$.
The article suggest two different ways of computing the confidence from the rating matrix via a linear or logarithmic transformation.
\begin{align*}
c_{u,i} = \left\{
 \begin{array}{@{}l@{\thinspace}l}
   1 + \alpha \cdot r_{u,i}\\
   1 + \alpha \cdot \log\left(1 + \frac{r_{u,i}}{\epsilon} \right)\\
 \end{array}
\right.
\end{align*}


\subsection{Hyperparameter space}
For all baseline algorithms and datasets, we determined the optimal parameters via Bayesian search \cite{antenucci2018artist} using the implementation of Scikit-Optimize\footnote{\url{https://scikit-optimize.github.io/}}.
We explored 50 cases for each algorithm, where the first 15 were used for the initial random points. Details on the hyperparameter space in Appendix \ref{sec:hyperparameter_range}.

\paragraph{Methodological note} The boundaries of the hyperparametes have been chosen by preferring them to be reasonably wide rather than small. If a certain hyperparameter was often found to be optimal at its highest or lowest interval, those boundaries were extended and the experiments repeated.

\subsection{Early stopping}
The number of epochs a ML or DL model should be trained for is another parameter, therefore we search for the optimal number of epochs as well, by optimizing the recommendation quality on the validation set.
As it is commonly done, we apply early stopping. When applying early stopping we use two different independent copies of the current model, one is the model that is still being trained, the other is the model with the best recommendation quality found so far. The first model is trained for a given number of epochs, followed by an evaluation step using the validation set. If the recommendation quality is better than the best one found so far, the best model is updated.
As it is commonly done, if the recommendation quality of the model does not improve over the best one for a certain number of epochs, the train stops before the maximum number of epochs is reached.
Due to how time consuming an evaluation step is, we run 5 train epochs before each validation step.
Moreover, we choose to early-stop the training if for 5 consecutive validation steps the recommendation quality of the model is worse than the best one found so far\footnote{This early stopping is consistent with what adopted by Keras, see \url{https://keras.io/callbacks/\#earlystopping}}. 
This condition is less strict than what applied for example by \cite{he2017neuralfactorizationmachines} \footnote{\url{https://github.com/hexiangnan/neural_factorization_machine/blob/master/NeuralFM.py}} where in the publicly available implementation is shown that the training stops only if for 5 consecutive epochs the recommendation quality on the validation set is monotonically getting worse.


\subsection{Training time and recommendations per second}
\label{sec:train_time}
We also compare the train time of different algorithms, baselines and DL algorithm. The purpose of this comparison is to provide a hint on how computationally intensive the different algorithms are.

We apply a similar methodology as \cite{vaswani2017attention} by reporting the computational cost of the different algorithms in terms of training time. \mf{check}

To ensure a fair comparison, while different sets of experiments may be run on different servers, we guarantee that the results reported on each table are obtained on the same machine with no other concurrent processes running. While it is true that DL algorithms have been developed to be used on GPUs and, therefore, running them on CPUs will result in them being much slower, this we argue it is not an unfair comparison since it helps to determine the magnitude of the different computational cost those methods have. It would be instead unfair to compare KNN algorithms able to run in a short amount of time on a CPU to a DL algorithm trained on an expensive GPU (e.g. in \cite{hu2018leveragingmetapathcontext} the authors state they have used 2 GTX 1080, which the official NVIDIA website at the time of writing quotes at a unit price of 570 euro).



For non personalised algorithms and the DL algorithm we report the train time of a single execution. For the personalised baselines requiring parameter tuning, we report the mean and standard deviation of the train time of all the hyper-parameters explored.
\emph{Train time} refers to the total time required for the training of the model, in case of algorithms applying early-stopping it includes all the evaluation time as that constitutes integral part of the training phase.
We also report the average and standard deviation of the time required to generate the recommendations for all users and the number of users per second recommendations can be generated for.
All times are reported in seconds. When a time interval is very big, we report it also using a bigger unit to ease the comparison.

\mf{mention something more about the implementation of the baselines?}
\paragraph{Factors that could impact the result} To make the comparison more transparent we stress that many factors independent from the algorithm being executed and its theoretical computational complexity may have an impact on the train and recommendation time. For example: the DL code provided by the authors may not be engineered to achieve the best computational efficiency and therefore will appear slower than what it could actually be; the availability of specific instruction sets (e.g. FMA, AVX2) on the servers may allow DL libraries like Tensoflow or Keras to run much faster, and so on.
We point out that all baseline algorithms are implemented by either exploiting native Python's numpy functions and vectorization (i.e. P3alpha, RP3beta, PureSVD) or developing an ad-hoc Cython module, for the most intensive computational tasks like the item-item similarity.

\paragraph{Computational resources used for DL algorithms}
Not all of them have presently been trained on gpu, resutls for CollaborativeDL are on CPU

For SIGIR, RecSys, KDD, WWW, IJCAI: Amazon instance p3.2xlarge, 8 vCPU, 30GB RAM, Tesla V100-SXM2-16GB, compute capability: 7.0, CUDA 10.

For AAAI, CIKM: Amazon instance p2.xlarge, 4 vCPU, 60MB RAM, Tesla K80, Compute Capability 3.7.


\subsection{Global computation cost}
In summary, the experiments here reported required the following computational load:
\begin{itemize}
    \item Algorithm - dataset experiments: 928
    \item Algorithm - dataset experiments with hyperparameter tuning: 41010
    \item Train time: 241.60 days (CPU and GPU)
    \item Train, validation and test time: 253.74 days (CPU and GPU)
\end{itemize}

The baselines required the following computational load:
\begin{itemize}
    \item Algorithm - dataset experiments: 876
    \item Algorithm - dataset experiments with hyperparameter tuning: 40762
    \item Train time: 204.00 days (CPU c3.4xlarge)
    \item Train, validation and test time: 215.65 days (CPU c3.4xlarge)
\end{itemize}

The DL algorithms required the following computational load:
\begin{itemize}
    \item Algorithm - dataset experiments: 52
    \item Algorithm - dataset experiments with hyperparameter tuning (SpectralCF only): 248
    \item Train time: 37.60 days (GPU p3.2xlarge)
    \item Train, validation and test time: 38.08 days (GPU p3.2xlarge)
\end{itemize}




\subsection{Useful references}
\emph{Hate Speech Detection is Not as Easy as You May Think: A Closer Look at Model Validation} \footnote{\url{https://dl.acm.org/citation.cfm?id=3331262}}



